Energy Patterns for Web: An Exploratory Study

As the energy footprint generated by software is increasing at an alarming rate, understanding how to develop energy-efficient applications has become a necessity. Previous work has introduced catalogs of coding practices, also known as energy patterns. These patterns are yet limited to Mobile or third-party libraries. In this study, we focus on the Web domain--a main source of energy consumption. First, we investigated whether and how Mobile energy patterns could be ported to this domain and found that 20 patterns could be ported. Then, we interviewed six expert web developers from different companies to challenge the ported patterns. Most developers expressed concerns for antipatterns, specifically with functional antipatterns, and were able to formulate guidelines to locate these patterns in the source code. Finally, to quantify the effect of Web energy patterns on energy consumption, we set up an automated pipeline to evaluate two ported patterns: 'Dynamic Retry Delay' (DRD) and 'Open Only When Necessary' (OOWN). With this, we found no evidence that the DRD pattern consumes less energy than its antipattern, while the opposite is true for OOWN. Data and Material: https://doi.org/10.5281/zenodo.8404487

==> tables/eng-patterns-motivation.tex <==
\begin{table*}[tbh]
	\begin{center}
		\caption{ Excerpts from Developers on their motivation for \eps and corresponding codes for the motivations}
		\label{tab:eng-patterns-motivation}
		\begin{tabular}{p{0.17\textwidth}p{0.5\textwidth}p{0.29\textwidth}}
  \toprule
  			\textbf{Developers} & \textbf{Excerpts} & \textbf{Codes} \\\midrule
     P1 (moderately concerned) & \emph{\EAPS correlates with efficiency and computational complexity.} & Efficiency, Complexity
\\
P5 (somewhat concerned)                           & \emph{It depends if its locally run, or on the cloud. If local, I don't really care. If GPUs are involved or the cloud, I am more concerned because I read about energy consumption of large data centers, and I know that GPUs consume a lot of power.}   &  Local computation, Cloud computation, GPU energy consumption \\
P6 (somewhat concerned) &
\emph{Application optimization and performance are still more important than energy optimization.}
& Optimization, Performance \\

 \hline
\end{tabular}
\end{center}
\end{table*}

==> tables/pattern-applicability.tex <==
\begin{table}
\begin{center}
\footnotesize
		\caption{Energy Patterns for the web domain with their applicability and classification to client (C) or Server(S)}
		\label{tab:patterns_applicability}
		\begin{tabular}{p{0.45\linewidth}p{0.18\linewidth}p{0.23\linewidth}}
  \toprule
  			\textbf{Pattern} &\textbf{Applicability} & \textbf{Client/Server-end}\\\midrule
\darkui				& \yes      & C    \\
\dynretdel          & \yes      & S    \\
\avoidextrawork     & \yes      & S    \\
\raceidle           & \yes      & S    \\
\openwneccesary     & \yes      & S    \\
\pushpoll           & \yes      & S    \\
\powersave          & partially & C    \\
\poweraware         & partially & C    \\
\reducesize         & \yes      & S    \\
\wificell           & \no       & -    \\
\suplog             & \yes      & S    \\
\batchoper          & \yes      & S    \\
\cache              & \yes      & S    \\
\decreaserate       & \yes      & S    \\
\usrknowbest        & \yes      & C    \\
\informusr          & partially & C    \\
\enoresolution      & \yes       & S    \\
\sensorfusion       & \no       & -    \\
\killtask           & \yes      & S    \\
\noscrinteraction	& partially & S    \\
\avoidgraphic 		& \yes      & S    \\
\mansyncod          & \yes      & S    \\
\hline
\end{tabular}
\end{center}
\end{table}

==> tables/patterns_description.tex <==
\begin{table*}[tbh]
\footnotesize
	\begin{center}
		\caption{ Mobile \eps by Cruz \etal \cite{cruz2019catalog} with their description }
		\label{tab:patterns_description}
		\begin{tabular}{p{0.17\linewidth}p{0.77\linewidth}}
  \toprule
  			\textbf{Pattern} & \textbf{Description}\\\midrule
\darkui                           & Provide a dark UI color theme to save battery on devices with AMOLED screens.                                                                          \\
\dynretdel                      & Whenever an attempt to access a resource fails, increase the time interval before retrying to access the same resource.                                 \\
\avoidextrawork                   & Avoid performing tasks that are either not visible, do not have a direct impact on the user experience to the user or quickly become obsolete.         \\
\raceidle                            & Release resources or services as soon as possible (such as wake locks, screen).                                                                        \\
\openwneccesary                 & Open/start resources/services only when they are strictly necessary.                                                                                   \\
\pushpoll                          & Use push notifications to receive updates from resources, instead of actively querying resources (i.e., polling).                                      \\
\powersave                          & Provide an energy efficient mode in which user experience can drop for the sake of better energy usage.                                                \\
\poweraware                          & Have a different behavior when the device is connected/disconnected to a power station or has different battery levels.                                \\
\reducesize                              & When transmitting data, reduce its size as much as possible.                                                                                           \\
\wificell                      & Delay or disable heavy data connections until the device is connected to a WiFi network.                                                               \\
\suplog                           & Avoid using intensive logging.                                                                                                                         \\
\batchoper                         & Batch multiple operations instead of putting the device into an active state many times.                                                              \\
\cache                                   & Avoid performing unnecessary operations by using cache mechanisms.                                                                                     \\
\decreaserate                            & Increase time between syncs/sensor reads as much as possible.                                                                                          \\
\usrknowbest                         & Allow users to enable/disable certain features in order to save energy.                                                                                \\
\informusr                             & Let the user know if the app is doing any battery-intensive operations.                                                                                \\
\enoresolution                        & Collect or provide high-accuracy data only when strictly necessary.                                                                                    \\
\sensorfusion                            & Use data from low-power sensors to infer whether new data needs to be collected from high-power sensors.                                               \\
\killtask                     & Provide means of interrupting energy greedy operations (e.g., using timeouts or user input).                                                         \\
\noscrinteraction                    & Whenever possible, allow interaction without using the display.                                                                                         \\
\avoidgraphic & Graphics and animations are really important to improve the user experience. However, they can also be battery intensive – use them with moderation.   \\
\mansyncod                 & Perform tasks exclusively when requested by the user.                                                                                                  \\ \hline
\end{tabular}
\end{center}
\end{table*}
